CO2 packing polymorphism under confinement in cylindrical nanopores

We investigate the effect of cylindrical nano-confinement on the phase behaviour of a rigid model of carbon dioxide using both molecular dynamics and well tempered metadynamics. To this aim we study a simplified pore model across a parameter space comprising pore diameter, CO2-pore wall potential and CO2 density. In order to systematically identify ordering events within the pore model we devise a generally applicable approach based on the analysis of the distribution of intermolecular orientations. Our simulations suggest that, while confinement in nano-pores inhibits the formation of known crystal structures, it induces a remarkable variety of ordered packings unrelated to their bulk counterparts, and favours the establishment of short range order in the fluid phase. We summarise our findings by proposing a qualitative phase diagram for this model.

==> tex_files/table_phases.tex <==
\begin{table*}[h]
\small
  \caption{\ An example of a caption to accompany a table}
  \label{table_phases}
  %\begin{tabular*}{1\textwidth}{@{\extracolsep{\fill}}lll}
  \begin{tabular*}{1\textwidth}{@{\extracolsep{\fill}}m{1cm}m{5cm}m{5cm}}
    \hline
    structure & configuration & angle distribution \\
    & & \tiny{r$_{cut}$ = 0.4 nm} \\
    \hline
    & & \\
    {\LARGE A} & \includegraphics[width=0.4\textwidth]{Images/table/Aimage.png} & \includegraphics[width=0.25\textwidth]{Images/table/Aangles.png} \\
    & & \\
    {\LARGE B} & \includegraphics[width=0.4\textwidth]{Images/table/Bimage.png} & \includegraphics[width=0.25\textwidth]{Images/table/Bangles.png} \\
    & & \\
    {\LARGE C} & \includegraphics[width=0.4\textwidth]{Images/table/Cimage.png} & \includegraphics[width=0.25\textwidth]{Images/table/Cangles.png} \\
    & & \\
    {\LARGE D} & \includegraphics[width=0.4\textwidth]{Images/table/Dimage.png} & \includegraphics[width=0.25\textwidth]{Images/table/Dangles.png} \\
    \hline
  \end{tabular*}
\end{table*}

